Program Synthesis by Type-Guided Abstraction Refinement

We consider the problem of type-directed component based synthesis where, given a set of (typed) components and a query type, the goal is to synthesize a term that inhabits the query. Classical approaches based on proof search in intuitionistic logics do not scale up to the standard libraries of modern languages, which span hundreds or thousands of components. Recent graph reachability based methods proposed for languages like Java do scale, but only apply to components over monomorphic data and functions: polymorphic data and functions infinitely explode the size of the graph that must be searched, rendering synthesis intractable. We introduce type-guided abstraction refinement (TYGAR), a new approach for scalable type-directed synthesis over polymorphic datatypes and components. Our key insight is that we can overcome the explosion by building a graph over abstract types which represent a potentially unbounded set of concrete types. We show how to use graph reachability to search for candidate terms over abstract types, and introduce a new algorithm that uses proofs of untypeability of ill-typed candidates to iteratively refine the abstraction until a well-typed result is found. We have implemented TYGAR in H+, a tool that takes as input a set of Haskell libraries and a query type, and returns a Haskell term that uses functions from the provided libraries to implement the query type. We have evaluated H+ on a set of 44 queries using a set of popular Haskell libraries with a total of 291 components. Our results demonstrate that H+ returns an interesting solution within the first five results for 33 out of 44 queries. Moreover, TYGAR allows H+ to rapidly return well-typed terms, with the median time to first solution of just 1.4 seconds.

==> algorithm.tex <==
\section{Type-Guided Abstraction Refinement}\label{sec:algo}

In this section we formally define our target language \corelang,
its type system, and the synthesis problem.
%
We then show how to use the framework of \emph{abstract interpretation} \TODO{cite?}
to define algorithmic type checking for \corelang,
and how re-casting type checking in this way 
allows us to easily parameterize the type checker by the desired level of detail,
leading to \emph{abstract typing} and the \emph{abstract synthesis problem}.
%
Finally we present the \tygar synthesis algorithm,
which solves a sequence of abstract synthesis problems with gradually increasing level of detail.
% For simplicity, in this section we focus on the \emph{first-order} setting.
% higher-order function support is discussed in \TODO{where?}

\subsection{The \corelang Language}\label{sec:algo:concrete}

\corelang is a simple first-order language with a prenex-polymorphic type system.
%
Syntax and concrete typing rules are shown in \autoref{fig:lang}.
%
Base types $B$ include type variables $\tau$,
as well as applications of a type constructor to zero or more base types $C\ \many{B}$;
hereafter, we use the notation $\many{X}$ to denote zero or more occurrences of a syntactic element $X$.
%
Types $T$ include base types and first-order function types (with base-typed arguments).
%
Syntactic categories $b$ and $t$ are the ground counterparts to $B$ and $T$ (\ie they contain no type variables).
%
\TODO{Should we keep lambdas in the language? Our terms only have one top-level abstraction.}
%
Our term language differentiates between variables $x$,
which have ground base types and are stored in the \emph{typing environment} $\Gamma$,
and components $c$, 
whose (poly-)types are stored in the \emph{component library} $\Lambda$.
%
$\Lambda$ also comes equipped with a well-formedness relation $\jwf{T}$, 
which intuitively means that all type constructors inside $T$ are correctly and fully applied;
well-formedness extends straightforwardly to polytypes and environments. 
%
A \emph{substitution} $\sigma$ is a mapping from type variables to base types.
%
We denote with $\sapp{\sigma}{T}$ an application of $\sigma$ to type $T$,
which is defined in a standard way.

The typing judgment $\jtyping{\Gamma}{e}{t}$ is only defined for ground types $t$.
%
Polymorphic components are instantiated into ground monotypes by the \textsc{Comp} rule,
which angelically picks ground base types to substitute 
for the universally-quantified type variables in the component signature.
%
This rule implicitly requires that $[\many{b/\tau}]T$ be ground,
which always holds as long as the component signature is closed (\ie contains no free type variables).
%
% Although we only present the declarative version of the type system,
% algorithmic type checking can be implemented using Hindley-Milner type inference.

% \TODO{Uncurry applications?}

\begin{figure}
\begin{minipage}{.45\textwidth}
\small
\textbf{Syntax}
$$
\begin{array}{llll}
% Terms    
% e &::= x \mid c \mid \eapp{e}{e}                         & \text{\emph{Terms}}\\  
e &::= x \mid c \mid \eapp{e}{e} \mid \elam{x}{e}        & \text{\emph{Terms}}\\  
% \\
% Types
b &::= C\ \many{b}                                       & \text{\emph{Ground Base Types}}\\  
t &::= b \mid b \to t                                    & \text{\emph{Ground Types}}\\  
B &::= \tau \mid C\ \many{B}                             & \text{\emph{Base Types}}\\  
T &::=  B \mid B \to T                                   & \emph{Types}\\  
P &::=  \many{\forall\tau}.T                             & \text{\emph{Polytypes}}\\
\Gamma &::=  \cdot \mid x:b,\Gamma                       & \text{\emph{Environments}}\\
\sigma &::=  [\many{B/\tau}]                             & \text{\emph{Substitutions}}
\end{array}
$$
\end{minipage}
%
\begin{minipage}{.45\textwidth}
\small
\textbf{Typing}\quad$\boxed{\jtyping{\Gamma}{e}{t}}$
\begin{gather*}
\inference[\textsc{T-Var}]
{\Gamma(x) = b}
{\jtyping{\Gamma}{x}{b} }
\\
\inference[\textsc{T-Comp}]
{\ty{c} = \many{\forall\tau}.T & \many{\jwf{b}}}
{\jtyping{\Gamma}{c}{\sapp{[\many{b/\tau}]}{T}} }
\\
\inference[\textsc{T-App}]
{ \jtyping{\Gamma}{e_1}{b \to t} &  
  \jtyping{\Gamma}{e_2}{b}}
{\jtyping{\Gamma}{\eapp{e_1}{e_2}}{t}}
\\
\inference[\textsc{T-Fun}]
{ \jtyping{\Gamma, x:b}{e}{t} }
{\jtyping{\Gamma}{\elam{x}{e}}{b \to t}}
\end{gather*}
\end{minipage}
\caption{\corelang: syntax and declarative type system.}\label{fig:lang}
\end{figure}

\mypara{Synthesis Problem}
%
A synthesis problem $(\Lambda, t)$ is a pair of a component library 
and \emph{query type} such that $\jwf{t}$.
%
We treat the query type as a monotype without loss of generality:
any query polytype $\many{\forall\tau}.T$ is equivalent to $[\many{C/\tau}]T$
where each $C$ is a fresh nullary type constructor.
%
A \emph{solution} to the synthesis problem is a program term $e$ such that $\jtyping{\cdot}{e}{t}$. 
%
Hereafter, we will only consider solutions in \emph{normal form} 
$\elam{x_1}{\ldots \elam{x_n}{e'}}$,
where $n$ is the arity of the query type and $e'$ is an \emph{application term},
\ie contains only variables and fully applied components%
\footnote{This does not restrict the solution space:
\corelang has no higher-order functions or recursion,
hence any well-typed program has an equivalent $\eta$-long $\beta$-normal form \TODO{cite?}.}.
%
The synthesis problem in \corelang in \emph{semi-decidable}:
if a solution $e$ exists, 
it can be found by enumerating programs in the order of increasing size;
the proof of undecidability can be found in \autoref{appendix:props}.


\subsection{Type Checking as Abstract Interpretation}

\TODO{Should we mention Cousot's ``Types as Abstract Interpretations'' somewhere?}
\TODO{How do we make type transformers generate fresh type variables every time?}

\mypara{Type subsumption lattice}
%
We say that type $T'$ \emph{is more specific than} type $T$, $T' \sub T$,
iff there exists $\sigma$ such that $\sapp{\sigma}{T} \equiv T'$
(where $\equiv$ is $\alpha$-equivalence).
%
Alternatively, we say that $T$ \emph{is more general than} or \emph{subsumes} $T'$.
%
It is easy to see that $\sub$ is a partial order on types.
%
For example, in a library with two nullary type constructors \T{A} and \T{B},
and a binary type constructor \T{P},
we have $\T{P A B} \sub \T{P _a B} \sub \T{P _a _b} \sub \tau$.

Let us augment the set of types with a special bottom type $\bot$ % ($\mathbf{B^*} = \mathbf{B} \cup \{\bot\}$)
that is strictly more specific than any other based type;
we also consider a bottom substitution $\sigma_{\bot}$ and define $\sapp{\sigma_{\bot}}{T} = \bot$ for any $T$.
%
We denote the \emph{most general unifier} (MGU) of $T_1$ and $T_2$ as $\mgu{T_1, T_2}$,
and define it to be $\sigma_{\bot}$ if $T_1$ and $T_2$ cannot be unified.
%
By slight abuse of notation we write $\mgu{\many{T_1, T_2}}$ for the MGU of a sequence of pairs of types,
where the MGU of an empty sequence is an empty substitution ($\mgu{\cdot} = []$).
%
The \emph{meet} of two base types is defined as $B_1 \meet B_2 = \sapp{\sigma}{B_1} (= \sapp{\sigma}{B_2})$,
where $\sigma = \mgu{B_1, B_2}$.
%
For example, $\T{P _a B} \meet \T{P A _b} = \T{P A B}$ while $\T{P _a B} \meet \T{P _b A} = \bot$.
%
The \emph{join} of two base types $B_1 \join B_2$ is the anti-unifier of $B_1$ and $B_2$.
%
For example, $\T{P A A} \join \T{P B B} = \T{P _a _a}$ while $\T{P A A} \join \T{B} = \tau$.

Let us denote $\basebots = \bases \cup \{\bot\}$ the set of base types augmented with $\bot$.
%
We can show that $\langle \basebots, \sub, \join, \meet \rangle$ is a \emph{lattice}
with bottom element $\bot$ and top element $\tau$;
in fact it is isomorphic to the well-known \emph{subsumption lattice} on first-order logic terms~\cite{plotkin1970lattice}.

% \mypara{Concretization function}
% %
% The \emph{concretization} of a base type $B \in \basebots$ is the set of its ground instances:
% $\gamma(B) = \{b \mid b \sub B\}$.
% %
% We can show that $T' \sub T$ iff $\gamma(T') \subseteq \gamma(T)$.
%
%
% Finally, $\gamma(\bot) = \emptyset$ while $\gamma(\T{P _a B})$ is the infinite set \setof{\T{P A B}, \T{P B B}, \T{P (P A A) B}, \T{P (P A B) B}, \ldots}.

\mypara{Type Transformers}
%
A component signature can be interpreted as a partial function
that maps (tuples of) ground types to ground types.
%
For example, intuitively, a component \T{l :: forall _b.L _b -> M _b} 
maps \T{L A} to \T{M A}, \T{L (M A)} to \T{M (M A)}, and \T{A} to $\bot$.
%
This gives rise to \emph{type transformer} semantics for components,
which is similar to predicate transformer semantics in predicate abstraction and SYNGAR~\cite{WangDS18},
but instead of being designed by a domain expert
can be derived automatically from the component signatures.

More formally, a \emph{type transformer} for a component $c$
where $\ty{c} = \many{\forall\tau} . \many{B_i} \to B$
is a function $\sem{c}_{\Lambda}\colon \many{\basebots} \to \basebots$ defined as follows:
$$
\sem{c}_{\Lambda}(\many{B'_i}) = \sapp{\sigma}{B} \quad\text{where}\ \sigma = \mgu{\many{B_i, B'_i}}
$$
%
We omit the subscript $\Lambda$ where the library is clear from the context.
%
For example, for the component \T{l} above:
$\sem{\T{l}}(\T{L (M _t)}) = \T{M (M _t)}$, 
$\sem{\T{l}}(\tau) = \T{M _b}$, 
and $\sem{\T{l}}(\T{A}) = \bot$ (because $\mgu{\T{L _b}, \T{A}} = \sigma_{\bot}$).
%
We can show that this type transformer is \emph{sound} in the sense that
in any concrete type derivation where the argument to \T{l} is an instance of some $B$,
its result is guaranteed to be an instance of $\sem{\T{l}}(B)$.
%
The transformer is also \emph{monotone} in the sense that applying it to more specific types
yield a more specific type.

\begin{lemma}[Soundness of Type Transformers]\label{lemma:trans-sound}
Let $c$ be a component such that $\ty{c} = \many{\forall\tau} . \many{B_i} \to B$.
For any types $\many{B'_i}$ and substitution $\sigma$, 
such that $\many{\sapp{\sigma}{B_i} \sub B'_i}$,
we have $\sapp{\sigma}{B} \sub \sem{c}(\many{B'_i})$.
\end{lemma}

\begin{lemma}[Monotonicity of Type Transformers]\label{lemma:trans-monotone}
For any component $c$ and any types $\many{B^1_i}$ and $\many{B^2_i}$, 
such that $\many{B^1_i \sub B^2_i}$,
we have $\sem{c}(\many{B^1_i}) \sub \sem{c}(\many{B^2_i})$.
\end{lemma}

\begin{figure}
% \begin{minipage}{.45\textwidth}
% \small
% \textbf{Type Inference}\quad$\boxed{\jtinfer{\Gamma}{e}{B}}$
% \begin{gather*}
% \inference[\textsc{I-Var}]
% {\Gamma(x) = b}
% {\jtinfer{\Gamma}{x}{b} }
% \\
% \inference[\textsc{I-App}]
% { \many{\jtinfer{\Gamma}{e_i}{B_i}} }
% {\jtinfer{\Gamma}{\eapp{c}{\many{e_i}}}{\sem{c}(\many{B_i})}}
% \end{gather*}
% \textbf{Type Checking}\quad$\boxed{\jtcheck{\Gamma}{e}{t}}$
% \begin{gather*}
% \inference[\textsc{C-Fun}]
% { \jtcheck{\Gamma, x:b}{e}{t} }
% {\jtcheck{\Gamma}{\elam{x}{e}}{b \to t}}
% \\
% \inference[\textsc{C-Base}]
% {\jtinfer{\Gamma}{e}{B} & b \sub B}
% {\jtcheck{\Gamma}{e}{b} }
% \end{gather*}
% \end{minipage}
% %
% \begin{minipage}{.45\textwidth}
\small
\textbf{(Abstract) Type Inference}\quad$\boxed{\jainfer{\Gamma}{e}{B}{\memph{\abset}}}$
\begin{gather*}
\inference[\textsc{I-Var}]
{\Gamma(x) = b}
{\jainfer{\Gamma}{x}{\memph{\alpha_{\abset}(\mnoemph{b})}}{\memph{\abset}} }
\quad\quad
\inference[\textsc{I-App}]
{ \many{\jainfer{\Gamma}{e_i}{B_i}{\memph{\abset}}} }
{\jainfer{\Gamma}{\eapp{c}{\many{e_i}}}{\memph{\alpha_{\abset}\left(\mnoemph{\sem{c}(\many{B_i})}\right)}}{\memph{\abset}}}
\end{gather*}
\textbf{(Abstract) Type Checking}\quad$\boxed{\jacheck{\Gamma}{e}{t}{\memph{\abset}}}$
\begin{gather*}
\inference[\textsc{C-Fun}]
{ \jacheck{\Gamma, x:b}{e}{t}{\memph{\abset}} }
{\jacheck{\Gamma}{\elam{x}{e}}{b \to t}{\memph{\abset}}}
\quad\quad
\inference[\textsc{C-Base}]
{\jainfer{\Gamma}{e}{B}{\memph{\abset}} & b \sub B}
{\jacheck{\Gamma}{e}{b}{\memph{\abset}} }
\end{gather*}
% \end{minipage}
\caption{Abstract type checking for \corelang. 
Treating $\alpha_{\abset}$ as the identity function yields concrete type checking.}\label{fig:abstract-typing}
\end{figure}

\mypara{Type Checking}
%
We can use type transformers to define algorithmic type checking for \corelang,
as shown in \autoref{fig:abstract-typing}.
%
For now, ignore the parts of the rules highlighted in red,
or, in other words, assume that $\alpha_{\abset}$ is the identity function;
the true meaning of this function is explained in the next section.
%
As is standard in bidirectional type checking~\cite{PierceTu00},
the type system is defined using two judgments:
the \emph{inference judgment} \jtinfer{\Gamma}{e}{B} generates the (base) type $B$ from the term $e$,
while the \emph{checking judgment} \jtcheck{\Gamma}{e}{t} checks $e$ against a known (ground) type $t$.
%
% We leverage the fact that \corelang is a first-order language
% and that any well-typed term has an equivalent $\eta$-long $\beta$-normal form,
% to only consider terms of the form $\elam{x_1}{\ldots \elam{x_n}{e'}}$,
% where $e'$ is an \emph{application term},
% \ie contains only variables and fully applied components.
%
Algorithmic typing assumes that the term is in normal form, as defined in \autoref{sec:algo:concrete}.
%
During type checking, the outer $\lambda$-abstractions are handled by the checking rule \textsc{C-Fun},
and then the type of inner application term is inferred 
and compared with the given type $b$ in \textsc{C-Base}.

The only interesting rule is the inference rule \textsc{I-App},
which handles (uncurried) component applications using their corresponding type transformers.
%
Nullary components are handled by the same rule
(note that in this case $\sem{c} = B$ where $\ty{c} = \many{\forall\alpha}.B$).
%
This type system is algorithmic, because we have eliminated the angelic choice of polymorphic component instantiations
(recall the \textsc{T-Comp} rule in the declarative type system).
%
Moreover, type inference for application terms can be thought of as abstract interpretation,
where the abstract domain is the type subsumption lattice:
for any application term $e$, the inference computes its ``abstract value'' $B$
(known in type inference literature as its \emph{most general type}).
%
\TODO{This sentence is strange, because for us the full TSL is the \emph{concrete} domain, not abstract.
How do we say this better?}
%
We can show that on terms in normal form, the algorithmic system is sound and complete \wrt the declarative one.

\begin{theorem}[Soundness and Completeness of Type Checking]\label{thm:algo-sound}
Let $e$ be a term in normal form.
For any ground type $t$, \jtyping{\cdot}{e}{t} iff \jtcheck{\cdot}{e}{t}.
\end{theorem}
\begin{proof}
Proof proceeds by induction on the derivation of \jtyping{\Gamma}{e}{t} and \jtcheck{\Gamma}{e}{t}
and uses lemmas that $\jtinfer{\Gamma}{e}{B} \Rightarrow \jtyping{\Gamma}{e}{b}$ for all $b \sub B$, 
and $\jtyping{\Gamma}{e}{b} \Rightarrow \jtinfer{\Gamma}{e}{B}$ for some $B \sqsupseteq b$.
\end{proof}


\subsection{Abstract Typing}

The algorithmic typing as presented so far is not particularly interesting:
it is pretty-standard Hindley-Milner type inference
(except it's simpler because the language is first-order and the top-level type is given,
so it never has to guess types of $\lambda$-binders).
%
However, casting type inference as abstract interpretation
gives us the flexibility to tune the \emph{precision} of the type system
by restricting the abstract domain to a sub-lattice of the full type subsumption lattice.
%
This is similar to predicate abstraction, 
where precision is tuned by restricting the abstract domain to boolean combinations of a finite set of predicates.

\mypara{Abstract Cover}
%
An \emph{abstract cover} $\abset = \{A_1, \ldots, A_n\}$ is a set of base types $A_i \in \basebots$
that contains $\tau$ and $\bot$, 
and is a sub-lattice of the type subsumption lattice (\ie is closed under its meet and join).
\TODO{We actually only care about closed under meet. But why?}
%
For example, in a library with a nullary constructor \T{A} and two unary constructors \T{L} and \T{M},
$\abset_0 = \{\tau, \bot\}$,
$\abset_1 = \{\tau, \T{A}, \T{L _t}, \bot\}$,
and $\abset_2 = \{\tau, \T{A}, \T{L _t}, \T{L (M _t)}, \T{M (M _t)}, \bot\}$
are abstract covers.
%
Note that in a cover, the scope of a type variable is each individual base type,
so the different instances of $\tau$ above are unrelated.
%
We say that an abstract cover $\abset'$ \emph{refines} a cover $\abset$ ($\abset' \refines \abset$)
if $\abset$ is a sub-lattice of $\abset'$.
%
In the example above, $\abset_2 \refines \abset_1 \refines \abset_0$.

\mypara{Abstraction function}
%
Given an abstract cover $\abset$, 
the \emph{abstraction} $\alpha_{\abset}\colon \basebots \to \basebots$ of a base type $B$
is defined as the most specific type in $\abset$ that subsumes $B$:
$$
\alpha_{\abset}(B) = A\in \abset\ \text{such that}\ B\sub A\ \text{and}\ \forall A'\in \abset.B\sub A'\Rightarrow A\sub A'
$$
We can show that $\alpha_{\abset}(B)$ is unique,
because $\abset$ is closed under meet.
%
\TODO{Should we explain how to compute it? Do we actually compute it efficiently, or just by iterating over $\abset$?}
%
In abstract interpretation, it is customary to define a dual \emph{concretization} function.
%
In our case, the abstract domain $\abset$ is a sub-lattice of the concrete domain $\basebots$,
and hence our concretization function is the identity function $\mathit{id}$.
%
It is easy to show that $\alpha_{\abset}$ and $\mathit{id}$ form a \emph{Galois insertion},
because $B \sub \mathit{id}(\alpha_{\abset}(B))$ and $A = \alpha_{\abset}(\mathit{id}(A))$
both hold by definition of $\alpha_{\abset}$.


\mypara{Abstract Type Checking}
%
Armed with the definition of abstraction function,
let us now revisit \autoref{fig:abstract-typing} and consider the highlighted parts we omitted previously.
%
The two abstract typing judgments---for checking and inference---are parameterized by the abstract cover. 
%
The only interesting changes are in the \emph{abstract type inference} judgment $\jainfer{\Gamma}{e}{B}{\abset}$,
which applies the abstraction function to the inferred type at every step.
%
For example, recall the covers $\abset_1$ and $\abset_2$ defined above,
and consider a term \T{l xs} where $\ty{\T{l}} = \forall \beta.\T{L}\ \beta \to \T{M}\ \beta$
and $\Gamma(\T{xs}) = \T{L (M A)}$.
%
Then in $\abset_1$ we infer \jainfer{\Gamma}{\T{l xs}}{\tau}{\abset_1},
since $\alpha_{\abset_1}(\T{L (M A)}) = \T{L _t}$
and $\sem{\T{l}}(\T{L _t}) = \T{M _t}$, but \T{M _t} is abstracted to $\tau$.
%
However, in $\abset_2$ we infer \jainfer{\Gamma}{\T{l xs}}{\T{M (M _t)}}{\abset_2},
since $\alpha_{\abset_2}(\T{L (M A)}) = \T{L (M _t)}$,
and $\sem{\T{l}}(\T{L (M _t)}) = \T{M (M _t)}$, which is abstracted to itself.

\begin{theorem}[Refinement]\label{thm:refine}
Typing with a refined cover is no less precise:
for any $\Lambda$, $\Gamma$, $e$, $t$, $\abset$, $\abset'$,
if $\abset' \refines \abset$
and $\jacheck{\Gamma}{e}{t}{\abset'}$
then $\jacheck{\Gamma}{e}{t}{\abset}$.
\end{theorem}


\begin{corollary}\label{thm:over-typecheck}
Abstract typing over-approximates concrete typing:
for any $\Lambda$, $\Gamma$, $e$, $t$, $\abset$,
if $\jtcheck{\Gamma}{e}{t}$
then $\jacheck{\Gamma}{e}{t}{\abset}$.
\end{corollary}
\begin{proof}
Follows from \autoref{thm:refine} because $\basebots \refines \abset$ for any $\abset$.
\end{proof}


\mypara{Abstract Synthesis Problem}
%
An abstract synthesis problem $(\Lambda, t, \abset)$ is a triple 
of a component library, query type, and abstract.
%
A \emph{solution} to the abstract synthesis problem is a program term $e$ such that $\jacheck{\cdot}{e}{t}{\abset}$. 

\begin{theorem}\label{thm:over}
A solution to a concrete synthesis problem is also a solution to any of its abstractions:
for any $\Lambda$, $\Gamma$, $t$, $\abset$, $e$,
if $e$ is a solution to $(\Lambda, t)$,
then it is also a solution to $(\Lambda, t, \abset)$.
\end{theorem}
\begin{proof}
Follows from \autoref{thm:over-typecheck} and \autoref{thm:algo-sound}.
\end{proof}


\subsection{Abstract Transition Nets}\label{sec:algo:atn}

Next we discuss how to construct an abstract transition net (ATN)
for a given abstract synthesis problem $(\Lambda, t, \abset)$,
and use ATN reachability to find a solution to this synthesis problem.

\mypara{Petri Nets}
%
A \emph{Petri net} $N$ is a triple $(P, T, E)$,
where $P$ is a set of places,
$T$ is the a set of transitions,
$E\colon (P\times T)\cup(T\times P)\to \nat$ is a matrix of edge multiplicities
(absence of an edge is represented by a zero entry).
%
A \emph{marking} of a Petri net is a mapping $M\colon P\to \nat$
that assigns a non-negative number of tokens to every place.
%
A \emph{transition firing} is a triple $M_1 \steps{t} M_2$,
such that for all places $p$: $M_1(p) \geq E(p, t) \wedge M_2(p) = M_1(p) - E(p, t) + E(t, p)$.
%
A sequence of transitions $t_1,\ldots,t_n$ is a \emph{path} between $M$ and $M'$
if $M \steps{t_1} M_1 \ldots M_{n - 1} \steps{t_n} M'$ is a sequence of transition firings.

\mypara{ATN Construction}
%
Consider an abstract synthesis problem $(\Lambda, t, \abset)$,
where $t = b_1 \to \ldots \to b_n \to b$.
% let $\args{S}$ be the sequence of argument types of $S$ and $\ret{S}$ be the return type of $S$.
%
An \emph{abstract transition net} $\net(\Lambda, t, \abset)$ is a triple $(N, \mathbf{M}, \mathbf{M'})$,
where $N$ is a Petri net, and $\mathbf{M}$, $\mathbf{M'}$ are sets of \emph{initial} and \emph{final} markings,
defined as follows:
\begin{enumerate}
\item the set of \emph{places} of $N$ is $\abset^{-} \triangleq \abset \setminus \setof{\bot}$;
\item \label{step:trans}
      for each component $c \in \Lambda$ 
      and for each tuple $A, A_1, \ldots, A_m \in \abset^{-}$, where $m$ is the arity of $c$,
      add a \emph{transition} $t$ iff $\alpha_{\abset}\left(\sem{c}(A_1, \ldots, A_m)\right) \equiv A$;
      set $E(t, A) = 1$ and add 1 to $E(A_j, t)$ for every $j \in (1, m)$;
\item a valid \emph{initial marking} $M \in \mathbf{M}$ 
      must have zero tokens everywhere except in $\alpha_{\abset}(b_i)$ for any $i \in (1, n)$;
\item a valid \emph{final marking} $M' \in \mathbf{M'}$ 
      assigns one token to a single place $A$, such that $b \sub A$.
% \item for each place $p \in \rng{\args{S}}$, 
      % we add a self-loop \emph{copy transition} $\kappa$, such that $W(p, \kappa) = 1$ and $W(\kappa, p) = 2$,
      % and a self-loop \emph{delete transition} $\delta$, such that $W(p, \delta) = 1$ and $W(\delta, p) = 0$.
\end{enumerate}

We will now highlight differences between our ATN construction and prior work on \sypet.
%
In the monomorphic setting of \sypet,
it is sufficient to add a single transition per component;
in the presence of polymorphic components, however, 
we need to add a transition for every \emph{abstract instance} of the component's polytype.
%
To compute the set of abstract instances, we consider all possible $m$-tuples of places,
and for each one compute the result of the abstract type transformer $\alpha_{\abset}\left(\sem{c}(A_1, \ldots, A_m)\right)$;
this result is either $\bot$, in which case no transition is added,
or some $A \in \abset^-$, in which case we add a transition from $A_1, \ldots, A_m$ to $A$.

Unlike \sypet, where the final marking contains a single token in the result type $b$, 
we must allow for several possible final markings:
we allow the token to end up in any place $A$ that subsumes $b$, 
not just in its most precise abstraction $\alpha_{\abset}(b)$.
%
This is because, like any abstract interpretation, 
abstract type inference might lose precision;
hence requiring that it infer the most precise type $\alpha_{\abset}(b)$ 
for the body of the solution would lead to incompleteness.

Finally, consider the set of initial markings:
in this section, we describe an ATN that implements a simple, structural type system,
where each function argument can be used zero or more times.
%
Hence we allow placing any non-negative number of tokens into each of $\alpha_{\abset}(b_i)$.
%
We can easily adapt the ATN definition to implement a relevant type system
by requiring at least one token in each $\alpha_{\abset}(b_i)$
(this is what our implementation does, see \autoref{sec:impl}).
%
A linear type system can be supported by requiring exactly one token per argument $i$
placed into $\alpha_{\abset}(b_i)$
(this reduces the set $\mathbf{M}$ to a singleton).


\mypara{From Paths to Programs}
%
Given an ATN $(N, \mathbf{M}, \mathbf{M'})$,
a path $\pi = [t_1, \ldots, t_n]$ is a \emph{valid path} of the ATN 
($\pi \models (N, \mathbf{M}, \mathbf{M'})$),
if it is a path from some $M \in \mathbf{M}$ to some $M' \in \mathbf{M'}$ in $N$.
%
Any valid path $\pi$
corresponds to a set of program terms $\fromPath{\pi}$.
%
The mapping from paths to programs has been defined in prior work on \sypet,
so we do not formalize it here;
intuitively, multiple programs arise 
because a path does not distinguish between different tokens in one place
and has no notion of order of incoming edges of a transition.
%
Importantly, $\fromPath{\pi}$
only generates terms in normal form.
%
% every term in $\fromPath{\pi}$ is of the form
% $\elam{x_1}{\ldots\ \elam{x_n}{e}}$,
% where $n$ is the number of tokens in the initial marking $M$,
% and $e$ consists only of variables $x_1 \ldots x_n$ and \emph{fully applied} components.


\begin{theorem}[Completeness of ATN Reachability]\label{thm:atn-complete}
For any $\Lambda$, $e$, $t$, $\abset$, $\pi$,
if $\jacheck{\cdot}{e}{t}{\abset}$ and $e \in \fromPath{\pi}$
then $\pi \models \net(\Lambda, t, \abset)$.
\end{theorem}

\begin{theorem}[Soundness of ATN Reachability]\label{thm:atn-sound}
For any $\Lambda$, $t$, $\abset$, $\pi$,
if $\pi \models \net(\Lambda, t, \abset)$,
then there exists $e$ such that $e \in \fromPath{\pi}$
and $\jacheck{\cdot}{e}{t}{\abset}$.
\end{theorem}

% \TODO{These theorems are nontrivial; 
% they should have been proved in Sypet, but weren't:
% they did not even have a type system there.}

\mypara{Abstract Synthesis Algorithm}
%
\autoref{alg:synthesis} (left) presents an algorithm
for solving an abstract synthesis problem $(\Lambda, t, \abset)$.
%
The algorithm first constructs the ATN $\net(\Lambda, t, \abset)$.
% 
Next, the function \textproc{\shortestpath} uses a constraint solver 
to find a shortest valid path $\pi \models \net(\Lambda, t, \abset)$%
\footnote{\autoref{sec:impl:encoding} details our encoding of ATN reachability into constraints.}.
%
From \autoref{thm:atn-complete}, 
we know that if no valid path exists (no final marking is reachable from any initial marking),
then the abstract synthesis program has no solution,
so the algorithm returns $\bot$.
%
Otherwise, it enumerates all programs $e \in \fromPath{\pi}$
and type-checks them abstractly,
until it encounters an $e$ that is abstractly well-typed
(such an $e$ must exists per \autoref{thm:atn-sound}).

\begin{figure}
\begin{minipage}{.45\textwidth}
  \small
  \begin{algorithmic}[1]
    \Require{Abstract synthesis problem ($\Lambda, t, \abset$)}
    \Ensure{Solution $e$ or $\bot$ if no solution}  
    \Statex
    \Function{\abssynth}{$\Lambda, t, \abset$}
      \Let{$(N, \mathbf{M}, \mathbf{M'})$}{$\net(\Lambda, t, \abset)$}
      \Let{$\pi$}{\Call{\shortestpath}{$N, \mathbf{M}, \mathbf{M'}$}}
      \If{$\pi = \bot$}
        \State \Return{$\bot$}
      \Else 
        \For{$e \in \fromPath{\pi}$}
          \If{$\jacheck{\cdot}{e}{t}{\abset}$}
            \State \Return{$e$}
          \EndIf
        \EndFor             
      \EndIf
      \Statex
    \EndFunction
  \end{algorithmic}
\end{minipage}
%
\begin{minipage}{.45\textwidth}
  \small
  \begin{algorithmic}[1]
    \Require{Synthesis problem ($\Lambda, t$), initial cover $\abset_0$}
    \Ensure{Solution $e$ or $\bot$ if no solution}  
    \Statex
    \Function{Synthesize}{$\Lambda, t, \abset_0$}
      \Let{$\abset$}{$\abset_0$}
      \While{true}
        \Let{e}{\Call{\abssynth}{$\Lambda, t, \abset$}}\label{algo:cand}
        \If{$e = \bot$}
          \State \Return{$\bot$}
        \ElsIf{$\jtcheck{\cdot}{e}{t}$}\label{algo:tc}
          \State \Return{$e$}
        \Else
          \Let{$\abset$}{\Call{Refine}{$\abset, e, t$}}
        \EndIf
      \EndWhile
    \EndFunction
  \end{algorithmic}
\end{minipage}  
\caption{(left) Algorithm for the abstract synthesis problem. 
(right) The \tygar algorithm.}\label{alg:synthesis}
\end{figure}


\subsection{The \tygar Algorithm}

We now turn to the core of our technique:
the \emph{type-guided abstraction refinement} (\tygar) algorithm.
%
The pseudocode is shown in \autoref{alg:synthesis} (right).
%
The algorithm takes as input a (concrete) synthesis problem $(\Lambda, t)$
and an initial abstract cover $\abset_0$,
and either returns a solution $e$ to the synthesis problem
or $\bot$ if $t$ cannot be inhabited using the components in $\Lambda$.
%
The general idea behind \tygar is to iteratively refine the current abstract cover $\abset$
(starting with $\abset_0$)
until it is specific enough that a solution to an abstract synthesis problem
is also well-typed in the concrete type system. 
%
In every iteration, \tygar first solves the abstract synthesis problem
at the current level of abstraction $\abset$,
using the previously defined algorithm \textproc{\abssynth}.
%
If the abstract problem has no solution,
then neither does the concrete one (by \autoref{thm:over}),
so the algorithm returns $\bot$.
%
Otherwise, the algorithm type-checks the term $e$ against the concrete query type.
%
If it is well-typed, then $e$ is the solution to the synthesis problem $(\Lambda, t)$;
otherwise $e$ is \emph{spurious}.

\mypara{Refinement}
%
The \emph{key step} in the \tygar algorithm is the procedure \textproc{Refine},
which takes as input the current cover $\abset$ and a spurious program $e$
and returns a refinement $\abset'$ of the current cover ($\abset' \refines \abset$)
such that $e$ is abstractly ill-typed in $\abset'$ ($\jnatyping{\cdot}{e}{t}{\abset'}$).
%
Procedure \textproc{Refine} is presented in detail in \autoref{sec:algo:refine},
but the declarative description above
is sufficient to see how it helps the synthesis algorithm make progress:
in the next iteration, \textproc{\abssynth} cannot return the same spurious program $e$,
since it no longer type-checks abstractly.
%
Moreover, the intuition is that along with $e$ the refinement rules out many other spurious programs
that are ill-typed ``for a similar reason''.

\mypara{Initial Cover}
%
The choice of initial cover $\abset_0$
has no influence on the correctness of the algoirthm.
%
A natural choice is the most general cover $\{\tau, \bot\}$.
%
In our experiments (\autoref{sec:eval})
we found that synthesis is more efficient if we pick the initial cover in such a way
that it represents the query type $t$ concretely.
%
Intuitively, the reason is that the distinctions between the types in $t$
are very likely to be important for solving the synthesis problem,
so there is no need to make the algorithm re-discover them from scratch.

\mypara{Formal Guarantees}
%
The procedure \textproc{Synthesize} is a sound and complete semi-algorithm 
for the synthesis problem in \corelang. 
% \TODO{is ``Complete'' a right word?}

\begin{theorem}[Soundness]
Any program the algorithm returns is well-typed:
for any $\Lambda, t, \abset_0$, if $\text{\textproc{Synthesize}}(\Lambda, t, \abset_0)$
returns $e \neq \bot$, then $\jtyping{\cdot}{e}{t}$.
\end{theorem}
\begin{proof}[Proof Sketch]
This follows trivially from the type check in line~\ref{algo:tc} of the algorithm.
\end{proof}

\begin{theorem}[Completeness]
If a solution exists, the algorithm will find one:
for any $\Lambda, t, \abset_0$, if there exists $e$ such that $\jtyping{\cdot}{e}{t}$
then $\text{\textproc{Synthesize}}(\Lambda, t, \abset_0)$
will terminate and return $e' \neq \bot$.
\end{theorem}
\begin{proof}[Proof Sketch]
Let $e_0$ be some shortest solution to $(\Lambda, t)$
and let $k$ be the number of all syntactically valid programs with as many or fewer components than $e_0$.
Line~\ref{algo:cand}
cannot return $\bot$ or a program $e$ that has more components than $e_0$,
since $e_0$ is abstractly well-typed at any $\abset$ by \autoref{thm:over-typecheck},
and \textproc{\abssynth} always returns a shortest abstractly well-typed program,
when one exists by \autoref{thm:atn-complete}.
Line~\ref{algo:cand} also cannot return the same solution twice
by the property of \textproc{Refine}.
Hence the algorithm must find a solution in at most $k$ iterations.
\end{proof}

When there is no solution, our algorithm might not terminate.
This is unavoidable, since the synthesis problem is only semi-decidable,
as we discussed in \autoref{sec:algo:concrete}.
%
In practice, we impose an upper bound on the length of the solution,
which then guarantees termination.


\subsection{Refining the Abstract Cover}\label{sec:algo:refine}

\begin{figure}
\begin{minipage}{.46\textwidth}
  \small
  \begin{algorithmic}[1]
    \Require{$\abset, e, T$, s.t. $\jntyping{\cdot}{e}{T}$}
    \Ensure{$\abset' \refines \abset$, s.t. $\jnatyping{\cdot}{e}{\alpha_{\abset'}(T)}{\abset'}$}  
    \Function{Refine}{$\abset, e, T$}
      \Let{$\Gamma,e',B,B'$}{\Call{Localize}{$e,T$}}
      \Let{$\abset'$}{\Call{Distinguish}{$B,B'$}}
      \Let{$A$}{$\intersect{\alpha_{\abset'}(B)}{\absTypeof{e'}}$}
      \Let{$\abset$}{\Call{Split}{$\abset, A, \absTypeof{e'}$}}
      \State \Return{\Call{Propagate}{$\abset, A, e'$}}
    \EndFunction
  \end{algorithmic}

  \begin{algorithmic}[1]
    \Statex
    \Require{$e, T$, s.t. $\jntyping{\cdot}{e}{T}$}
    \Ensure{$\Gamma,e',B,B'$, s.t. $\jtyping{\Gamma}{e'}{B'}$ but $\nunifies{B}{B'}$}  
    \Function{Localize}{$e, T$}
      \State standard bottom-up type inference on $e$
    \EndFunction
    \Statex
  \end{algorithmic}  

  \begin{algorithmic}[1]
    \Statex
    \Require{$B, B'$, s.t. $\nunifies{B}{B'}$}
    \Ensure{$\abset$, s.t. $\nunifies{\alpha_{\abset}(B)}{\alpha_{\abset}(B')}$}
    \Function{Distinguish}{$C\ \many{B}, C\ \many{B'}$}
      \State{$(B_i, B'_i) \gets \many{(B, B')}$ s.t. $\nunifies{B_i}{B'_i}$}
      \Let{$\abset$}{\Call{Distinguish}{$B_i, B'_i$}}\label{algo:distinguish-recurse}
      \Let{$\abset$}{$\{C\ (\{\many{*}, A, \many{*}\}) \mid A \in \abset\}$}
      \State \Return{$\abset$}
    \EndFunction
    \Function{Distinguish}{$\abset, C\ \_, \_$}
      \State \Return{$\{C\ \T{*}, !C\}$}\label{algo:distinguish-base}
    \EndFunction
  \end{algorithmic}

  \begin{equation*}
    \begin{aligned}
      &\intersect{C\ \many{A}}{C\ \many{B}}   = C\ \many{\intersect{A_i}{B_i}}\\
      &\intersect{!\many{C}}{C_1\ \many{A}} = C_1\ \many{A}\ \text{if}\ C_1\ \not\in \many{C}\\
      &\intersect{!\many{C_1}}{!\many{C_2}}   = \ !\many{C_1 \cup C_2}\\
      &\intersect{\_}{\_}                     = \bot\\
    \end{aligned}
  \end{equation*}
\end{minipage}
%
\begin{minipage}{.52\textwidth}
  \small
  \begin{algorithmic}[1]
    \Require{$\abset, A, A'$, s.t. $\unifies{A}{A'}$, $A \in \abset$ but $A' \not\in \abset$}
    \Ensure{$\abset' \refines \abset$, s.t. $A \not\in \abset'$ and $A' \in \abset'$} 
    \Function{Split}{$\abset, C\ \many{A}, C\ \many{A'}$}
      \For{$(A_i, A'_i) \in \many{(A, A')}$}
        \If{$\nunifies(A_i, A'_i)$}
          \Let{$\abset_i$}{\Call{Split}{$\peeli{\abset}{C}{i}, A_i, A'_i$}}\label{algo:split-recurse}
        \EndIf
        \Let{$\abset_i$}{$\{C\ (\many{A_{1, \cdots, i-1}}, A, A_{i+1}, \cdots\}) \mid A \in \abset_i\}$}
        \Let{$\abset$}{$\abset \setminus \{C\ \many{A}\} \cup \abset_i$}
      \EndFor
      \State \Return{$\abset$}
    \EndFunction
    \Function{Split}{$\abset, !\many{C}, C_1\ \many{A}$}
      \For{$A_i \in \many{A}$}
        \Let{$\abset_i$}{\Call{Split}{$\peeli{\abset}{C}{i}, *, A_i$}}\label{algo:split-comp-c}
        \Let{$\abset_i$}{$\{C\ (\{\many{A_{1, \cdots, i-1}}, A, \many{*}\}) \mid A \in \abset_i\}$}
        \Let{$\abset$}{$\abset \cup \abset_i$}
      \EndFor
      \Let{$\abset$}{$\abset \setminus {!\many{C}} \cup \{!(\tops{\abset} \cup {C_1})\}$}
      \State \Return{$\abset$}
    \EndFunction
    \Function{Split}{$\abset, !\many{C_1}, !\many{C_2}$}
      \For{$C_i \in \many{C_2}$}
        \If{$C_i \not\in \many{C_1}$}
          \Let{$\abset$}{\Call{Split}{$\abset, !\many{C_1}, C_i\ *$}}\label{algo:split-comp}
        \EndIf
      \EndFor
      \State \Return{$\abset$}    
    \EndFunction
  \end{algorithmic}

  \begin{algorithmic}[1]
    \Statex
    \Require{$\abset, A, e$, s.t. $A\in \abset$ and $\nunifies{A}{\typeof{e}}$}
    \Ensure{$\abset' \refines \abset$, s.t. $\jnatyping{\alpha_{\abset'}(\Gamma)}{e}{A}{\abset'}$}  
    \Function{Propagate}{$\abset, A, x$}
      \State \Return{$\abset$}\label{algo:prop:var}
    \EndFunction
    \Function{Propagate}{$\abset, A, c\ e_1\ \ldots\ e_n$}
      \Let{$(\many{\forall \tau}.B_1 \to \ldots \to B_n \to B)$}{$\ty{c}$}
      \Let{$\sigma$}{\Call{Unify}{B, A}}\label{algo:prop:unify}
      \If{$\sigma \neq \bot$}
        \For{$i \in 1..n$}
          \Let{$A_i$}{$\sigma[B_i]$}
          \Let{$A_i'$}{$\intersect{A_i}{\absTypeof{e_i}}$}
          \Let{$\abset$}{\Call{Split}{$\abset, A_i, A_i'$}}
          \Let{$\abset$}{\Call{Propagate}{$\abset, A_i, e_i$}}
        \EndFor             
      \EndIf
      \State \Return{$\abset$}
    \EndFunction
  \end{algorithmic}
\end{minipage}  
\caption{Refinement algorithm.}\label{alg:refinement}
\end{figure}

This section details the refinement step of the \tygar algorithm.
%
The pseudocode is given in \autoref{alg:refinement}.
%
The top-level function \textproc{Refine}($\abset, e, T$)
takes as inputs an abstract cover $\abset$, a term $e$, and a goal type $T$,
such that $e$ is ill-typed concretely ($\jntyping{\cdot}{e}{T}$),
but well-typed abstractly ($\jatyping{\cdot}{e}{\alpha_{\abset}(T)}{\abset}$).
%
It produces a refinement of the cover $\abset' \refines \abset$, 
such that $e$ is ill-typed abstractly in that new cover ($\jnatyping{\cdot}{e}{\alpha_{\abset'}(T)}{\abset'}$).
%
At a high level, \textproc{Refine} localizes a single concrete type error inside $e$
and makes sure that the new abstract cover $\abset'$ is discriminative enough
to detect that error.

\mypara{Error localization}
%
As the first step, \textproc{Refine} invokes the function \textproc{Localize}
that performs bottom-up Hindley-Milner type inference on $e$,
solving unification constraints as they are being generated.
%
Since we know that $e$ is ill-typed at $T$,
at some point during type inference the inferred type $B'$ of a subterm $e'$ of $e$ 
must fail to unify with its \emph{goal type} $B$
(which is either $\ret{T}$ if $e' = e$ or a parameter type of some component otherwise).
%
At this point, \textproc{Localize} returns a tuple of four: $\Gamma, e', B, B'$,
where $\Gamma$ is the current typing environment.
%
Note that because $e$ is in $\eta$-long $\beta$-normal form (as explained in \autoref{sec:algo:atn}),
we know that $\Gamma$ contains all the query parameters ($\Gamma = \many{x_i : B_i}$ where $\many{B_i} = \args{T}$),
the goal type $B$ is a base type,
and $e'$ contains only variables $x_i$ and fully-applied components.

\mypara{Distinguishing ununifiable types}
With a type error at hand, \textproc{Refine} invokes the function \textproc{Distinguish},
which weakens the expected type $B$ and its corresponding real type $B'$ 
to get the most general abstraction cover that discriminates them.
%
\textproc{Distinguish} takes as inputs 
the concrete expected type $B$ and the concrete real type $B'$,
such that $\nunifies{B}{B'}$;
it returns a cover $\abset$ such that $\nunifies{\alpha_{\abset}(B)}{\alpha_{\abset}(B')}$.
%
If two types have the same outermost constructor, it recurses into 
one of their arguments (line~\ref{algo:distinguish-recurse}),
packs the results back into the constructor $C$ and fill other arguments as \T{*}.
%
Otherwise, if $B$ starts with $C$ and $B'$ does not,
it introduces a distinction between $C\ \T{*}$ and $\tneg{C}$ into the cover (line~\ref{algo:distinguish-base}).

Although we find a partition of the universal type set that differs our 
ununifiable types, it may have different abstraction semantic from the current one.
For example, our current abstraction cover is 
$\abset = \{\T{L\ (M\ *), L\ !M, !L}\}$.
When we try to distinguish $\T{L (L a)}$ from $\T{L a}$, 
we choose the cover $\abset' = \{\T{L\ (L\ *), L\ !L}\}$,
where the type $\T{L\ (L\ a)}$ is abstracted as $\T{L\ !M}$ and $\T{L\ (L\ *)}$ 
respectively in two covers. In this case,
we compute the type intersection between them to merge the information 
on both sides by calling function $\intersect{}{}$.
Notice that we can always successfully compute the type intersection: 
the soundness of our algorithm ensures that the abstraction of the 
real type (i.e. $\absTypeof(e)$) covers the expected concrete type, and
we are doing intersection between two abstract types of the same concrete one,
which is impossible to be empty.

\mypara{Splitting a cover}
After distinguishing the found type error, \textproc{Refine} invokes the function
\textproc{Split} to refine the current cover $\abset$
so that it discriminates between $\absTypeof{e'}$ and the intersection type $A$.
%
\textproc{Split} takes as inputs a cover $\abset$, two abstract types $A, A'$
where $A'$ is the subtype of $A$ and only $A$ is included in the cover $\abset$.
It returns a refinement $\abset'$ of $\abset$, where the new cover contains $A'$ but not $A$.
%
If the two types share the outermost constructor $C$, it recurses into the 
arguments (line~\ref{algo:split-recurse}),
and uses the resulting split to refine those $\abset$ entries that start with $C$ incrementally.
%
If only one of the types is a complementary type, it recurses into 
the arguments of the other constructor $C_1$ refining all the types in $\abset$ 
that start with $C$ incrementally.
At last, it remove the old complementary type and add $!(\tops{\abset} \cup \{C_1\})$ into $\abset$ (line~\ref{algo:split-comp-c}).
%
If both of the types are complementary type, it adds their difference into the
$\abset$ one by one and removes the old complementary type (line~\ref{algo:split-comp}).

%
\mypara{Propagating the goal type}
Finally, \textproc{Refine} invokes \textproc{Propagate}
to propagate the new abstract goal $A$ 
back through the subterms of $e'$.
%
\textproc{Propagate} takes as inputs a cover $\abset$, an abstract base type $A \in \abset$
and a well-typed term $e$ whose concrete type does not unify with $A$.
%
Its goal is to refine the cover $\abset$ into $\abset'$
so that $e$ is abstractly ill-typed at $A$ in $\abset'$.
%
If $e$ is a variable (line~\ref{algo:prop:var}), no further refinement is necessary.
%
However, if $e$ is an application $c\ e_1\ \ldots\ e_n$ 
of a polymorphic component $c$ of type $\many{\forall \tau}.B_1 \to \ldots \to B_n \to B$,
we cannot yet guarantee that $e$ is abstractly ill-typed at $A$.
%
The reason is that the \textsc{Comp} rule of abstract type checking 
is free to pick a \emph{different instance} of $c$ than the one used by concrete type checking;
hence we need to make sure that \emph{no} instance of $c$ that works for the goal type $A$,
also works for its arguments $e_1\ \ldots\ e_n$.
%
To that end, we unify $A$ with $c$'s return type $B$ (line~\ref{algo:prop:unify})
to effectively compute all instances that work for $A$.
%
If this unification fails, then propagation is complete.
%
Otherwise, if unification results in a substitution $\sigma$,
for each argument $i$, we compute its goal type $A_i$ as $\sigma[B_i]$,
intersect between the expected type and the real type as $A_i'$,
split the cover to make it discriminate between $A_i$ and $A_i'$,
and recurse.

\mypara{Example}
%
Let us walk through the refinement step in iteration 2 of our running example from \autoref{sec:examples:abstract}.
%
Our query type is $T = \T{a -> L (M a) -> a}$
and the spurious program is $e = \lambda x_1\ x_2 . f\ x_1\ (l\ x_2)$,
where $\ty{f} = \forall \alpha . \alpha \to \T{M}\ \alpha \to \alpha$
and $\ty{l} = \forall \beta . \T{L}\ \beta\to \T{M}\ \beta$.
Our current abstract cover is $\abset = \{\T{L *}, \T{!L}\}$,
so it is easy to check that $e$ is ill-typed concretely but well-typed abstractly.
%
\textproc{Localize}$(e,T)$ returns $\Gamma = \{x_1:\T{a}, x_2:\T{L (M a)}\}$,
$e' = l\ x_2$ and $B = \T{M a}$,
since $e'$ is the subterm of $e$ that is well-typed on its own,
but its type \T{M (M a)} does not unify with the goal type $B$
imposed by the parameter type of $f\ x_1$. So we find a weakest cover
$\abset' = \{\T{M (M *), M !M}\}$ to distinguish them. 
Under $\abset'$, we compute the intersection between $\T{!L}$ and $\T{M !M}$ to
get the expected abstract type $\T{M !M}$.
%
Next, we refine $\abset$ so that the abstract type of $e'$ is distinguished
from the abstract goal type by calling \textproc{Split}$(\abset,\ \T{!L},\ \T{M !M})$,
which yields $\abset = \{\T{M (M *)}, \T{M !M}, \T{L *}, \T{!LM}\}$.
%
Now we need to propagate the new abstraction of $B$, $\T{M !M}$,
back through $e'$.

To this end, we invoke \textproc{Propagate}$(\abset, \T{M !M}, l\ x_2)$.
%
Since $l$ is a polymorphic component, we unify its return type with the goal,
\textproc{Unify}$(\T{M}\ \beta, \T{M !M})$ yielding $\sigma = [\beta\mapsto \T{!M}]$.
%
Applying this substitution to the argument type yields \T{L !M},
which shares its abstraction, \T{L *}, with the actual type of the argument \T{L (M a)}.
%
Hence we split the \T{L *} entry in the current abstraction into \T{L (M *)} and \T{L !M},
yielding $\abset = \{\T{M (M *)}, \T{M !M}, \T{L (M *)}, \T{L !M}, \T{!LM}\}$.
%
At this point, propagation reached a variable ($x_2$), 
hence the process is complete.
%
Indeed, our new cover is such that $e$ is abstractly ill-typed.

\mypara{Example Again}
%
Let us see the another example with higher-kinded type constructor \T{Pair}.
%
Our query type is $T = \T{P a b -> P (P a b) (P b a))}$
and the spurious program is $e = \lambda x . Pair\ (Just\ (snd\ x))\ (fst\ x)$,
where $\ty{Just} = \forall \alpha . \alpha\ \to \T{M}\ \alpha$,
$\ty{fst} = \forall \alpha\ \beta . \T{P}\ \alpha\ \beta \to \alpha$
and $\ty{snd} = \forall \alpha\ \beta . \T{P}\ \alpha\ \beta \to \beta$.
Our current abstract cover is $\abset = \{\T{P * (P * *)}, \T{M *}, \T{P * !P}, \T{!PM}\}$,
so it is easy to check that $e$ is ill-typed concretely but well-typed abstractly.
%
\textproc{Localize}$(e,T)$ returns $\Gamma = \{x:\T{P a b}\}$,
$e' = e$, $B = \T{P (P a b) (P b a)}$ and $B' = \T{P (M b) a}$,
since $e'$ has the type \T{P (M b) a} does not unify with the goal type $B$. 
So we find a weakest cover
$\abset' = \{\T{P (P * *), P !P *}\}$ to distinguish them. 
Under $\abset$ and $\abset'$, we compute the intersection 
between $\T{P * (P * *)}$ and $\T{P (P * *) *}$ to
get the expected abstract type $\T{P (P * *) (P * *)}$.
%
Next, we refine $\abset$ so that the abstract type of $e'$ is distinguished
from the abstract goal type by calling \textproc{Split}$(\abset,\ \T{P * (P * *)},\ \T{P (P * *) (P * *)})$,
which yields $\abset = \{\T{P (P * *) (P * *)}, \T{P !P (P * *)}, \T{M *}, \T{P * !P}, \T{!PM}\}$,
%
Now we need to propagate the new abstraction of $B$, \T{P (P * *) (P * *)},
back through $e'$.

Then, we invoke \textproc{Propagate}$(\abset, \T{P (P * *) (P * *)}, e')$.
By unifying this abstract type with \T{P} $\alpha$ $\beta$ which is the return
type of the pair constructor, we get the unifier $\sigma = [\alpha\mapsto \T{P * *}, \beta \mapsto \T{P * *}]$.
Applying the substitution to the arguments, we get that both of the arguments are \T{P * *}.

To this end, we invoke \textproc{Propagate} recursively on both arguments of the outermost pair constructor.
It is obvious that on the first argument, the propagation gets stuck. Here, we only focus on the second argument, where
we call \textproc{Propagate}$(\abset, \T{P * *}, fst\ x)$.
%
Since $fst$ is also a polymorphic component, we unify its return type with the goal,
\textproc{Unify}$(\T{P}\ \alpha, \T{P * *})$ yielding $\sigma = [\alpha\mapsto \T{P * *}]$.
%
Applying this substitution to the argument type yields \T{P (P * *)} $\beta$, 
which contains the free type variable $\beta$, we can always view free type variables
as \T{*} because they can be any type. But in the bottom-up type checking, we tag
this node with abstract type \T{P * !P} so we see overlapping between these two,
by intersecting them together and then split the \T{P * !P} into \T{P (P * *) !P}
in the current abstraction, 
yielding $\abset = \{\T{P (P * *) (P * *)}, \T{P !P (P * *)}, \T{M *}, \T{P (P * *) !P}, \T{P !P !P}, \T{!PM}\}$.
%
Again, we invoke \textproc{Propagate}$(\abset, \T{P (P * *) !P}, x)$, we reached a variable ($x$),
hence the process is complete.
%
In our new cover, the program $e$ is abstractly ill-typed.

% \TODO{Compare with SYNGAR?}


==> curated.tex <==
\begin{figure}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}\hline
      N & Name & Query & Expected Solution & Rank\\
      \hline
      1 & intToByteString	& Int64 $\rightarrow$ ByteString	& \texttt{$\lambda$x. toLazyByteString (int64BE x)} & 3\\
      \hline
      2 & conjunctionMaybes	& [Maybe Bool] $\rightarrow$ Bool & \texttt{$\lambda$mbs. and (catMaybes mbs)} & >5\\
      \hline
      3 & firstJust &	a $\rightarrow$ [Maybe a] $\rightarrow$ a	& \texttt{$\lambda$x xs. fromMaybe x (listToMaybe (catMaybes xs))} & 1 \\
      \hline
      4 & both & (a $\rightarrow$ b) $\rightarrow$ (a, a) $\rightarrow$ (b, b)	& \texttt{$\lambda$f p. (f (fst p), f (snd p))}  & 1\\
      \hline
      5 & guaranteedRight	& Either a b $\rightarrow$ (a $\rightarrow$b) $\rightarrow$ b & \texttt{$\lambda$x f. either f id x} & 1 \\
      \hline
      6 & mbMap	& (a $\rightarrow$ Maybe b) $\rightarrow$ [a] $\rightarrow$ Maybe b & \texttt{$\lambda$f xs. listToMaybe (mapMaybe f xs)} & >5 \\
      \hline
      \end{tabular}
  }
  \caption{The six curated queries. Rank is how far down the expected solution appears among programs produced by \tool.}
  \label{fig:curated}
\end{figure}


==> quality.tex <==
\begin{figure}
  \resizebox{\textwidth}{!}{
  \input{quality_data}
  }
\caption{\tool quality results.
The first column is the query.
The next three columns describe the time to find the first solution.
The next three columns are the total time to produce the five solutions.
The numeric columns next to the solutions count the number of interesting solutions
for that experiment.
\TODO[Update this for the current table.]
}\label{fig:quality_results}
\end{figure}

==> scratch.tex <==

Type-directed synthesis and code completion: SyPet, InSynth, CodeHunt (no polymorphism).
Synquid, Djinn, MagicHaskeller? (do not scale to large APIs).
Type-directed search: Hoogle (no snippets).

Synthesis by abstraction refinement: Blaze.

CEGAR for Petri Nets.

% synth from tests     (pbe)
% synth from contracts (synquid, euphony, sketch, blaze)

\mypara{Type Inhabitation} %-- (djinn, insyth, perelman,rehof) 

\mypara{Graph Reachability} %-- (sypet, prospector) 

\mypara{CEGAR for Petri Nets} %-- (ganty, kloos)

\mypara{Dynamic Traces} % (codehint, matchmaker) 

\mypara{Probabilistic Models} % syhth from prob models  (slang, bayou)

PBE (tests)



\textbf{\sypet}

\mypara{Synquid}
Program synthesis based on refinement types \cite{PolikarpovaKS16} enables
synthesis of recursive functional programs by using refinement types
\cite{VazouSJVJ14}. The user defines a set of functions with refinement types
and specifies a hole they would like the system to synthesis code for. It works
through a new ``round-trip'' type checking process. The type checker works down
the type of hole and propogates refinement constraints down. The constraints
guide an enumerative search. It does not build a representation of the search
space and so it cannot prune uninhabited types early or group terms that share a
refinement type. Consequently, the system will not handle many components well as
it will have to enumeratively check them.

\mypara{Djinn}
Authored by Lennart Augustsson, \djinn is a theorem prover written in Haskell
that produces code snippets from a query and a set of component functions. The
tool uses intuitional propositional
logic CITATION NEEDED to build a proof using the available components that 
some composition exists to transtion between the input and output types. 
Importantly, \djinn has no relevancy requirement of its snippets. 
Additionally with no inherent understanding of lists, \djinn 
requires a user to define a set of list components, including 
an empty list constructor. 

These two facets of the system mean that many functions whose desired type is a list
can be trivially fulfilled by returning an empty list. By the nature of proof searches, we do not expect
\djinn to scale particularly well to hundreds of components.

